MaxFusion: Plug&Play Multi-Modal Generation in Text-to-Image Diffusion Models

Large diffusion-based Text-to-Image (T2I) models have shown impressive generative powers for text-to-image generation as well as spatially conditioned image generation. For most applications, we can train the model end-toend with paired data to obtain photorealistic generation quality. However, to add an additional task, one often needs to retrain the model from scratch using paired data across all modalities to retain good generation performance. In this paper, we tackle this issue and propose a novel strategy to scale a generative model across new tasks with minimal compute. During our experiments, we discovered that the variance maps of intermediate feature maps of diffusion models capture the intensity of conditioning. Utilizing this prior information, we propose MaxFusion, an efficient strategy to scale up text-to-image generation models to accommodate new modality conditions. Specifically, we combine aligned features of multiple models, hence bringing a compositional effect. Our fusion strategy can be integrated into off-the-shelf models to enhance their generative prowess.

==> metrics/alt_metrics.tex <==


\begin{table*}[!t]
\begin{center}
\setlength{\tabcolsep}{10pt}
\scalebox{0.8}{
\begin{tabular}{l l | c c c c c| c c c c c}
\toprule[0.15em]
%\rowcolor{color3} 
   && \multicolumn{5}{c|}{\textbf{CelebA dataset}} & \multicolumn{5}{c}{\textbf{FFHQ dataset}}  \\
\cline{2-12}
%\rowcolor{color3} 
   \textbf{Type}&\textbf{Method} & FID$\textcolor{black}{\downarrow}$ & LPIPS$\textcolor{black}{\downarrow}$& SSIM$\textcolor{black}{\uparrow}$ & MAE$\textcolor{black}{\uparrow}$  & F1~$\textcolor{black}{\uparrow}$ &  FID$\textcolor{black}{\downarrow}$ & LPIPS$\textcolor{black}{\downarrow}$& SSIM$\textcolor{black}{\uparrow}$ & MAE$\textcolor{black}{\uparrow}$  & F1~$\textcolor{black}{\uparrow}$   \\
\midrule[0.15em]
\multirow{5}{*}{Fine-Tuning} &SPADE\cite{park2019SPADE} &131.91 & 0.638 & 0.316 & 0.605&0.694 & 91.77& 0.624 & 0.340 & 0.649&0.728\\
&OASIS\cite{oasis}  & 118.67 & 0.624 & 0.318 & 0.579&0.663 & 99.94 &0.634 & 0.320 & 0.625&0.704 \\
&PIX2PIXHD\cite{wang2018pix2pixHD}& 153.19 & 0.611 & 0.282 & 0.716&0.819 & 223.85& 0.670 & 0.265 & 0.666&0.775  \\
&INADE\cite{tan2021diverse} &125.43& 0.632 & 0.279 & 0.881&0.932 & 134.11 & 0.656& 0.274 & 0.869&0.922 \\
% &DDPM\cite &111.35& 0.786 & 0.255 & 0.824&0.881 & 109.29& 0.703& 0.258 & 0.835&0.901 \\
\midrule[0.15em]
\multirow{5}{*}{Alternate} &SPADE\cite{park2019SPADE} & 89.29 & \textbf{0.523} & 0.376 & 0.890&0.936 & 75.73& \textbf{0.545} & 0.373 & 0.876&0.921\\
&OASIS\cite{oasis}  & 71.20 & 0.571 & 0.323 & 0.792&0.870 & 75.57 &0.593 & 0.331 & 0.786&0.863 \\
&PIX2PIXHD\cite{wang2018pix2pixHD}& 73.32 & 0.512 & 0.373 & 0.872&0.925 & 138.30& 0.560 & 0.363 & 0.840&0.898  \\
&INADE\cite{tan2021diverse} &54.27& 0.552  & 0.332& 0.887&0.933 & 47.40& 0.574 & 0.334  & 0.862&0.910\\
% &DDPM &55.23& 0.663  & 0.368&0.909&0.947 & 72.94& 0.681 & 0.365& 0.909&0.942  \\
\midrule[0.15em]
% \midrule[0.1em]


&TediGAN\cite{xia2021tedigan} &69.51 & 0.4823 & 0.417 & 0.834&0.905 & 125.27& 0.545 & 0.409&0.813 & 0.887\\
&OURS &\textbf{26.09} & 0.519 & \textbf{0.416} & \textbf{0.911}&\textbf{0.948} & \textbf{33.60}& 0.542 & \textbf{0.421}&\textbf{0.919} & \textbf{0.950} \\


\bottomrule[0.1em]
\end{tabular}}
\caption{Quantitative results for semantic labels to face generation on CelebA and FFHQ datasets. The alternate training based strategy and fine-tuning based training strategy are shown in the corresponding sections. $(\uparrow)$/  $(\downarrow)$ represents higher/ lower the metric lower the metrics, the better respectively. 
}
\label{table:semantic}
\end{center}
\vspace{-2em}
\end{table*}

==> metrics/interpolation.tex <==
\begin{figure}[tb!]
    \centering
    \setlength{\tabcolsep}{0.5pt}
    {\small
    \renewcommand{\arraystretch}{0.5} 
    \begin{tabular}{c c c c c c c c c c  }
    \captionsetup{type=figure, font=scriptsize}
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{Text
} }}
  \includegraphics[width=0.135\linewidth]{/sample3/text_unc/1.0_0.0_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/text_unc/1.0_0.2_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/text_unc/1.0_0.4_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/text_unc/1.0_0.5_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/text_unc/1.0_0.6_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/text_unc/1.0_0.8_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/text_unc/1.0_1.0_0.jpg}
\tabularnewline
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{Class}
}}
  \includegraphics[width=0.135\linewidth]{/sample3/class_unc/0.0_0.0_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/class_unc/0.0_0.2_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/class_unc/0.0_0.4_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/class_unc/0.0_0.5_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/class_unc/0.0_0.6_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/class_unc/0.0_0.8_0.jpg}
\includegraphics[width=0.135\linewidth]{/sample3/class_unc/0.0_1.0_0.jpg}
\tabularnewline
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{Mix
}}}
  \includegraphics[width=0.135\linewidth]{/sample3/our_unc/1.0_0.0_0.jpg}
  \includegraphics[width=0.135\linewidth]{/sample3/our_unc/1.0_0.2_0.jpg}
  \includegraphics[width=0.135\linewidth]{/sample3/our_unc/1.0_0.4_0.jpg}
  \includegraphics[width=0.135\linewidth]{/sample3/our_unc/1.0_0.5_0.jpg}
  \includegraphics[width=0.135\linewidth]{/sample3/our_unc/1.0_0.6_0.jpg}
  \includegraphics[width=0.135\linewidth]{/sample3/our_unc/1.0_0.8_0.jpg}
  \includegraphics[width=0.135\linewidth]{/sample3/our_unc/1.0_1.0_0.jpg}
\tabularnewline
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{Text
} }}
  \includegraphics[width=0.135\linewidth]{/samples5/text_unc/1.0_0.0_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/text_unc/1.0_0.2_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/text_unc/1.0_0.4_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/text_unc/1.0_0.5_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/text_unc/1.0_0.6_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/text_unc/1.0_0.8_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/text_unc/1.0_1.0_0.jpg}
\tabularnewline
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{Class}
 }}
 \includegraphics[width=0.135\linewidth]{/samples5/class_unc/0.0_0.0_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/class_unc/0.0_0.2_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/class_unc/0.0_0.4_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/class_unc/0.0_0.5_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/class_unc/0.0_0.6_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/class_unc/0.0_0.8_0.jpg}
\includegraphics[width=0.135\linewidth]{/samples5/class_unc/0.0_1.0_0.jpg}
\tabularnewline
    \raisebox{0.1in}{\rotatebox{90}{\small \emph{Mix
} }}
  \includegraphics[width=0.135\linewidth]{c/1.0_0.0_0.jpg}
  \includegraphics[width=0.135\linewidth]{c/1.0_0.2_0.jpg}
  \includegraphics[width=0.135\linewidth]{c/1.0_0.4_0.jpg}
  \includegraphics[width=0.135\linewidth]{c/1.0_0.5_0.jpg}
  \includegraphics[width=0.135\linewidth]{c/1.0_0.6_0.jpg}
  \includegraphics[width=0.135\linewidth]{c/1.0_0.8_0.jpg}
  \includegraphics[width=0.135\linewidth]{c/1.0_1.0_0.jpg}

\tabularnewline

    \tabularnewline
  $\scriptsize{Text}\xrightarrow[\text{weighing factor}]{\hspace*{2cm}}\scriptsize{Class}$

\vspace{2mm}
\vspace{-2\baselineskip}
\end{tabular}}
\vspace{-0.4cm}
\hspace{20pt}\captionof{figure}{\textbf{Interpolation across multiple modalities.} Here, \textit{\{class $\rightarrow$Text\}} denotes to where the unconditional model comes from.}
\label{fig:glideablation2}
\vspace{-2mm}
\end{figure}%

==> metrics/metrics_2modal1.tex <==
\begin{table}[t]
\centering

\scalebox{0.7}{
\begin{tabular}{c|c|c c c c c }
\toprule
Method&Modality&FID$(\downarrow)$&NIQE$(\downarrow)$&Clip$(\uparrow)$&Depth$(\downarrow)$&HED$(\downarrow)$\\
\midrule
PITI-Sketch\cite{liu2022compositional}&\emph{Uni} &38.50 &6.22 &0.2669 &0.0298&0.0417\\
\midrule
T2I-Adapter\cite{mou2023t2i}&\emph{Multimodal}  &30.63&3.90&\cellcolor{blue!25}0.2964 &0.0417 &0.1055  \\
Ours&\emph{Multimodal}&\cellcolor{blue!25}29.71  &\cellcolor{blue!25}2.86&0.2879 &\cellcolor{blue!25}0.0191 &\cellcolor{blue!25}0.0735 \\

\bottomrule
\end{tabular}
}
\caption{\textbf{Qualitative comparisons for $\{Hed, Depth \rightarrow Image\}$.} Quantitative results for different models for multimodal generation}
\label{tab:compgen1}
\vspace{-1mm}
\end{table}


==> metrics/unimulti.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.250\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{ablation/new_input/122.jpg}
      \includegraphics[width=1\linewidth]{ablation/new_input/1015.jpg}
      \caption{Label}
    \end{subfigure}
    % \begin{subfigure}[t]{0.250\linewidth}
    %   \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
    %   \includegraphics[width=1\linewidth]{ablation/hair/122.jpg}
    %   \includegraphics[width=1\linewidth]{ablation/hair/1015.jpg}
    %   \caption{Hair}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.250\linewidth}
    %   \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
    %   \includegraphics[width=1\linewidth]{ablation/face/122.jpg}
    %   \includegraphics[width=1\linewidth]{ablation/face/1015.jpg}
    %   \caption{Face}
    % \end{subfigure}
    \begin{subfigure}[t]{0.250\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{122.jpg}
      \includegraphics[width=1\linewidth]{1015.jpg}
      \caption{Combined}
    \end{subfigure}
    \begin{subfigure}[t]{0.250\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{ablation/our/122.jpg}
      \includegraphics[width=1\linewidth]{ablation/our/1015.jpg}
      \caption{OURS}
    \end{subfigure}
    \vspace{-3mm}    \caption{A visualization of generated images with combined conditional generation (uni-modal) with ours (multi-modal).  }
    \label{fig:ablation}
    \vspace{-2mm}
  \end{figure}


==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> tex_files/seg_depth.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{results/depth_hed/hed/000000185802.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/hed/000000019221.jpg}
      
      \includegraphics[width=1\linewidth]{results/seg_hed/hed/000000357748.jpg}


      \includegraphics[width=1\linewidth]{results/depth_seg/depth/000000005992.jpg}



    %   \includegraphics[width=1\linewidth]{/input_new/1035.jpg}
      \caption{TASK-1}
    \end{subfigure}
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{results/depth_hed/depth/000000185802.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/seg/000000019221.jpg}
      
      \includegraphics[width=1\linewidth]{results/seg_hed/seg/000000357748.jpg}

      \includegraphics[width=1\linewidth]{results/depth_seg/seg/000000005992.jpg}




    %   \includegraphics[width=1\linewidth]{/spade/1035.jpg}
      \caption{TASK-2\cite{park2019SPADE}}
    \end{subfigure}
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}

      \includegraphics[width=1\linewidth]{results/depth_hed/piti_seg/000000185802.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/spade/000000019221.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/spade/000000357748.jpg}

      \includegraphics[width=1\linewidth]{results/depth_seg/spade/000000005992.jpg}

      % \includegraphics[width=1\linewidth]{results/seg_hed/spade/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/pix2pixhd/1035.jpg}
      \caption{MultiControlNet\cite{wang2018pix2pixHD}}
    \end{subfigure}
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}

      \includegraphics[width=1\linewidth]{results/depth_hed/piti_sk/000000185802.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/piti/000000019221.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/piti/000000357748.jpg}

      \includegraphics[width=1\linewidth]{results/depth_seg/piti/000000005992.jpg}


      % \includegraphics[width=1\linewidth]{results/seg_hed/piti/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/inade/1035.jpg}
      \caption{MultiT2I-Adapter\cite{tan2021diverse}}
    \end{subfigure}
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}

      \includegraphics[width=1\linewidth]{results/depth_hed/adapter/000000185802.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/adapter/000000019221.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/adapter/000000357748.jpg}

      \includegraphics[width=1\linewidth]{results/depth_seg/adapter/000000005992.jpg}


      % \includegraphics[width=1\linewidth]{results/seg_hed/adapter/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/ddpm/1035.jpg}
      \caption{Unicontrol\cite{ho2020denoising}}
    \end{subfigure}
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{results/depth_hed/control/000000185802.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/control/000000019221.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/control/000000357748.jpg}

      \includegraphics[width=1\linewidth]{results/depth_seg/control/000000005992.jpg}



      % \includegraphics[width=1\linewidth]{results/seg_hed/control/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/tedigan/1035.jpg}
      \caption{SPADE\cite{xia2021tedigan}}
    \end{subfigure}
    \begin{subfigure}[t]{0.137\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{results/depth_hed/ours/000000185802.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/ours/000000019221.jpg}
      \includegraphics[width=1\linewidth]{results/seg_hed/ours/000000357748.jpg}

      \includegraphics[width=1\linewidth]
{results/depth_seg/ours/000000005992.jpg}


      % \includegraphics[width=1\linewidth]{results/seg_hed/ours/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/1035.jpg}
      \caption{OURS}
    \end{subfigure}
    \vspace{-3mm}    \caption{\textbf{Qualitative comparisons for semantic to face generation.} In this case, a single model is trained by alternating different input datasets across different iterations. During Inference time all the modalities are taken from a single dataset and the proposed sampling technique is used.}
    \label{fig:facesematic}
  \end{figure*}

==> tex_files/variance_intra.tex <==
\begin{figure*}[tb!]
    \centering
    \setlength{\tabcolsep}{0.5pt}
    {\small
    \renewcommand{\arraystretch}{0.5} 
    \begin{tabular}{c c c c c c c c c c c c c c }
    \captionsetup{type=figure, font=scriptsize}
    \includegraphics[width=0.105\linewidth]{varaince/132.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/spider_pose.jpg}
  % \includegraphics[width=0.105\linewidth]{varaince/pose_maps/0.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/pose_maps/1.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/pose_maps/2.jpg}
  % \includegraphics[width=0.105\linewidth]{varaince/luffy_pose/3.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/pose_maps/4.jpg}
  % \includegraphics[width=0.105\linewidth]{varaince/luffy_pose/5.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/pose_maps/6.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/pose_maps/7.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/pose_maps/8.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/pose_maps/9.jpg}
 % \hspace{0.5mm}
  \tabularnewline
  \includegraphics[width=0.105\linewidth]{varaince/131.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/spider-canny.jpg}
  % \includegraphics[width=0.105\linewidth]{varaince/canny_maps/0.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/canny_maps/1.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/canny_maps/2.jpg}
  % \includegraphics[width=0.105\linewidth]{varaince/anthlercanny/3.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/canny_maps/4.jpg}
  % \includegraphics[width=0.105\linewidth]{varaince/anthlercanny/5.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/canny_maps/6.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/canny_maps/7.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/canny_maps/8.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/canny_maps/9.jpg}
  \tabularnewline
  \includegraphics[width=0.105\linewidth]{varaince/133.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/spider_depth.jpg}
  % \includegraphics[width=0.105\linewidth]{varaince/depth_maps/110.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/depth_maps/111.jpg}

  % \includegraphics[width=0.105\linewidth]{varaince/flower_depth/1.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/depth_maps/112.jpg}
  % \includegraphics[width=0.105\linewidth]{varaince/flower_depth/3.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/depth_maps/114.jpg}
  % \includegraphics[width=0.105\linewidth]{varaince/flower_depth/5.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/depth_maps/116.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/depth_maps/117.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/depth_maps/118.jpg}
  \includegraphics[width=0.105\linewidth]{varaince/depth_maps/119.jpg}
  \tabularnewline

% {\small\hspace{15pt}Tibetan terrier\hskip10pt Teddy bear \hskip15pt Triceratops \hskip15pt Tree frog \hskip15pt Otterhound \hspace{20pt}Tibetan terrier\hskip10pt Teddy bear \hskip15pt Triceratops \hskip20pt Tree frog \hskip20pt Otterhound }\\
\vspace{-2mm}
\vspace{-2\baselineskip}
\end{tabular}}
% \vspace{-0.8cm}
\hspace{20pt}\captionof{figure}{Variance Maps across channels for Intermediate features of controlNet for conditions derived from the same image, Given the same text prompt and noise seed. Th variance map  has high values where the condition is present in these case as well}\label{fig:sup1b}
% \vspace{-8mm}
\end{figure*}%

==> tookits.tex <==

\usepackage{multirow}
\usepackage{booktabs}
\usepackage{subcaption}
\usepackage{amsmath,amsfonts,bm,amsthm,amssymb}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{graphics,graphicx,caption,float,color}
\usepackage{wrapfig}
\usepackage{bbm}
\usepackage{appendix}

% custom
\usepackage{listings}
\usepackage{xspace}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 
\usepackage{hhline}
\usepackage{multicol}
\usepackage{booktabs} 
\usepackage{makecell} % Xhline


% name of our model
\newcommand{\ffn}{TODO Our Method Name}
\newcommand{\ourabbr}{AdaptFormer\xspace}

\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\definecolor{MyDarkBlue}{rgb}{0,0.08,1}
\definecolor{MyDarkGreen}{rgb}{0.02,0.6,0.02}
\definecolor{MyDarkRed}{rgb}{0.8,0.02,0.02}
\definecolor{MyDarkOrange}{rgb}{0.40,0.2,0.02}
\definecolor{MyPurple}{RGB}{111,0,255}
\definecolor{MyRed}{rgb}{1.0,0.0,0.0}
\definecolor{MyGold}{rgb}{0.75,0.6,0.12}
\definecolor{MyDarkgray}{rgb}{0.66, 0.66, 0.66}

\definecolor{Image}{RGB}{93,59,155}
\definecolor{Video}{RGB}{105,145,60}

\definecolor{ice}{RGB}{84,146,214}
\definecolor{fire}{RGB}{217,129,63}
\definecolor{baselinecolor}{gray}{.9}
\definecolor{poscolor}{RGB}{212,17,89}
\definecolor{negcolor}{RGB}{26,133,255}
\definecolor{bestcolor}{RGB}{238, 255, 238}
% copy-paste from Kaiming's MAE, used for ablation tables
\newcolumntype{x}[1]{>{\centering\arraybackslash}p{#1pt}}
\newcolumntype{y}[1]{>{\raggedright\arraybackslash}p{#1pt}}
\newcolumntype{z}[1]{>{\raggedleft\arraybackslash}p{#1pt}}
% \newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize} % original style from MAE
% \newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering}%\footnotesize


\newcommand{\baseline}[1]{\cellcolor{baselinecolor}{#1}}
\newcommand{\bestcell}[1]{\cellcolor{bestcolor}{#1}}
\newcommand{\aaa}[1]{\textcolor{poscolor}{\small (#1)}}
\newcommand{\bbb}[1]{\textcolor{negcolor}{\small (#1)}}

\newcommand{\rebuttal}[1]{#1}
% \newcommand{\rebuttal}[1]{\textcolor{blue}{#1}}

\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\etal}{\emph{et.al.,}}


